DAG Learning on the Permutahedron

We propose a continuous optimization framework for discovering a latent directed acyclic graph (DAG) from observational data. Our approach optimizes over the polytope of permutation vectors, the so-called Permutahedron, to learn a topological ordering. Edges can be optimized jointly, or learned conditional on the ordering via a non-differentiable subroutine. Compared to existing continuous optimization approaches our formulation has a number of advantages including: 1. validity: optimizes over exact DAGs as opposed to other relaxations optimizing approximate DAGs; 2. modularity: accommodates any edge-optimization procedure, edge structural parameterization, and optimization loss; 3. end-to-end: either alternately iterates between node-ordering and edge-optimization, or optimizes them jointly. We demonstrate, on real-world data problems in protein-signaling and transcriptional network discovery, that our approach lies on the Pareto frontier of two key metrics, the SID and SHD.

==> figures/sem.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}[c]{0.2\textwidth}
  \begin{tikzpicture}[scale=0.8]

 
  \node[circle] (A) at (-8,-2) [draw, minimum width=0.5cm,minimum height=0.5cm] {$x_2$};
  
  \node[circle] (B) at (-6.5,-2) [draw, minimum width=0.5cm,minimum height=0.5cm] {$x_1$};
  
  \node[circle] (C) at (-6.5,-0.5) [draw, minimum width=0.5cm,minimum height=0.5cm] {$x_4$};
  
  \node[circle] (D) at (-5, -2) [draw, minimum width=0.5cm,minimum height=0.5cm] {$x_3$};
   
  
    \foreach \from/\to in {A/B, B/C, B/D, A/C}
\draw [->] (\from) -- (\to);

  \end{tikzpicture}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.7\textwidth}\centering \scalebox{0.8}{
  $\underbrace{\begin{pmatrix}
    0 & 0 & 2.5 & -0.5 \\
    1.3 & 0 & 0 & 0.3 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 0 & 0 \\
\end{pmatrix}}_{\rmA(\params)} = \underbrace{\begin{pmatrix}
    1.3 & 0.5 & 2.5 & -0.5 \\
    1.3 & -2. & 0 & 0.8 \\
    0.3 & 0 & 1.4 & 0 \\
    0.9 & 5.7 & 0 & 2.7 \\
\end{pmatrix}}_{\rmS(\params)} \circ \underbrace{\begin{pmatrix}
    0 & 0 & 1 & 1 \\
    1 & 0 & 1 & 1 \\
    0 & 0 & 0 & 0 \\
    0 & 0 & 1 & 0 \\
\end{pmatrix}}_{\rmM_{_{\sigma(\params)}}} \quad \underbrace{\begin{pmatrix} 1 \\ 0 \\ 3 \\ 2 \end{pmatrix}}_{\sigma(\params)}$} 
\end{subfigure}
  
  \caption{\textbf{Left:} True DAG with 4 nodes. \textbf{Right:} Our approach.}
\label{fig:causal_graph}
% \vspace{-0.15in}
\end{figure}


